Visualizing Movement Control Optimization Landscapes

A large body of animation research focuses on optimization of movement control, either as action sequences or policy parameters. However, as closed-form expressions of the objective functions are often not available, our understanding of the optimization problems is limited. Building on recent work on analyzing neural network training, we contribute novel visualizations of high-dimensional control optimization landscapes; this yields insights into why control optimization is hard and why common practices like early termination and spline-based action parameterizations make optimization easier. For example, our experiments show how trajectory optimization can become increasingly ill-conditioned with longer trajectories, but parameterizing control as partial target states---e.g., target angles converted to torques using a PD-controller---can act as an efficient preconditioner. Both our visualizations and quantitative empirical data also indicate that neural network policy optimization scales better than trajectory optimization for long planning horizons. Our work advances the understanding of movement optimization and our visualizations should also provide value in educational use.

==> figures_at_the_end.tex <==
%!TEX root = main.tex





==> scrapped.tex <==
For any $1 \ge c > 0$, lemma 4.23 of \cite{vempala2005random} bounds the probability of the norm being lower than a limit as

\begin{equation}
P\Bigg(||\mathbf{u}_{[:k]}|| < c \sqrt{\frac{k}{d}}\Bigg) \le (2c)^k. \label{eq:vempala}
\end{equation}




\section{Proof of Proposition 2}
Deriving the exact formula for the condition number of the 2D slice as a function of $d$ is beyond the scope of this paper. However, the visualization will display the ill-conditioning if one of the projection norms $||\mathbf{u}_{[:k]}||, ||\mathbf{v}_{[:k]}||$ differ from each other, i.e., $f(\mathbf{x})$ grows faster when moving along one axis than the other. Such vector pairs and all their rotations around $\mathbf{u} \times \mathbf{v}$ form good visualization basis vectors. Thus, we need to prove that randomly selecting such a pair becomes less probable with a large $d$. Assume that one first selects $\mathbf{u}$ randomly and then calculates $\mathbf{v}$ through orthogonalization as:

\begin{equation}
\mathbf{v}=\frac{\mathbf{r} - \mathbf{u} (\mathbf{u}^T\mathbf{r})}{||\mathbf{r} - \mathbf{u} (\mathbf{u}^T\mathbf{r})||},
\end{equation}

where $\mathbf{r} $ is another random unit-length vector independent of $\mathbf{u}$. With a large $d$, $\mathbf{u}$ and $\mathbf{r}$ are more likely to be orthogonal to begin with such that $\mathbf{u}^T\mathbf{r} \approx 0$ and $\mathbf{v} \approx \mathbf{r}$, which means that the norms $||\mathbf{u}_{[:k]}||, ||\mathbf{v}_{[:k]}||$ are independent random variables with the same expectation. Conversely, with small $d$, the orthogonalization has a larger effect, and affects the norm of $\mathbf{v}_{[:k]}$, making it more likely that the norms differ. For example, consider the case of $k=2$. If $\mathbf{u}$ is parallel to the subspace, i.e., lies in the plane spanned by the first two unit vectors, orthogonalization will rotate $\mathbf{v}$ away from the plane unless $\mathbf{r}$ is also parallel to the plane $\qed$ \textcolor{green}{CHECK: is this logic sound?}




